TrendFact: A Benchmark Towards Hotspot Perception in Automatic Fact-Checking

With the surge of online misinformation, Large Language Models (LLMs) and Reasoning Large Language Models (RLMs) serving as Automatic Fact-Checking (AFC) systems have emerged as a prominent paradigm for reliable, explainable verification. However, our empirical study reveals that this paradigm faces a critical risk asymmetry challenge when deployed in the real world under resource-constrained environments. While Hotspot Perception Ability (HPA), the capacity to dynamically allocate reasoning resources based on social impact, is essential to mitigate this risk, existing benchmarks lack the social metadata and evaluation framework to meet this urgent evaluation needs, thereby hindering the advancement of these AFC systems. To bridge this gap, we introduce TrendFact, the first benchmark capable of evaluating HPA and three fact-checking tasks. It consists of 7,643 curated samples sourced from trending platforms and professional datasets, with an evidence library containing 366,634 entries. To enable HPA assessment, we propose two novel metrics: the Explanation Consistency Score (ECS) to evaluate the reliability of verification reasoning, and the Hotspot Claim Perception Index (HCPI) to quantify the overall HPA of AFC systems. Extensive experiments demonstrate that existing AFC systems exhibit limited performance on TrendFact. Furthermore, our proposed FactISR framework effectively enhances HPA and computational efficiency for RLMs-served AFC systems.

==> revision_record.tex <==
二、写作与表达上的改进点
1. 术语与缩写
RLM 出现很晚才定义。

ECS/HCPI 在引入时没有解释。

一些缩写长时间不用后没有重新解释。

�� 改进建议：

在第一次出现缩写时写全称。

每个 Section 开头重新提醒重要缩写。

2. 论文结构与清晰度
表述冗余、逻辑不清。

关键定义太晚出现。

多个地方需要重写（审稿人一致建议“proofreading and restructuring”）。

�� 改进建议：

在引言里提前定义所有核心概念。

重组段落，让 dataset → metrics → method → experiments 逻辑更紧凑。

请同事或语言服务帮助润色。

3. 图表和附录说明不足
Figure captions 太简略，不知道怎么读。

Table 4 表现不佳，但正文没有解释清楚。

附录中的 Figure 引用错误（e.g., L763）。

�� 改进建议：

补充说明图表如何解读。

解释为什么 FactISR 在 Table 4 下表现差。

检查并修正引用错误。

4. 语言与格式问题
多处语法错误（“consistancy” → “consistency”等）。

不恰当的用词（“Chinese scenario” → “Chinese language”）。

引文前缺少空格。

软件和模型引用格式不规范。

�� 改进建议：

全文系统性 proofreading。

修正拼写、语法和标点。

格式化模型/工具名称并添加脚注或参考文献。
